CKnowEdit: A New Chinese Knowledge Editing Dataset for Linguistics, Facts, and Logic Error Correction in LLMs

Chinese, as a linguistic system rich in depth and complexity, is characterized by distinctive elements such as ancient poetry, proverbs, idioms, and other cultural constructs. However, current Large Language Models (LLMs) face limitations in these specialized domains, highlighting the need for the development of comprehensive datasets that can assess, continuously update, and progressively improve these culturally-grounded linguistic competencies through targeted training optimizations. To address this gap, we introduce CKnowEdit, the first-ever Chinese knowledge editing dataset designed to correct linguistic, factual, and logical errors in LLMs. We collect seven types of knowledge from a wide range of sources, including classical texts, idioms, and content from Baidu Tieba Ruozhiba, taking into account the unique polyphony, antithesis, and logical structures inherent in the Chinese language. By analyzing this dataset, we highlight the challenges current LLMs face in mastering Chinese. Furthermore, our evaluation of state-of-the-art knowledge editing techniques reveals opportunities to advance the correction of Chinese knowledge. Code and dataset are available at https://github.com/zjunlp/EasyEdit.

==> Table/case_study.tex <==
\begin{table*}[ht]
{
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{3pt}
\small
\begin{center}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{ll}
\toprule
\hline
\multirow{5}*{\textbf{Edit Success}}
& \textbf{Prompt:} \includegraphics[height=0.32cm]{figures/case_study1.png} 
( Please explain the meaning of ‘\includegraphics[height=0.32cm]{figures/wang.png}’ in ‘\includegraphics[height=0.32cm]{figures/shidongzhiwangri.png}’ ) \\
& \textbf{Target:} \includegraphics[height=0.28cm]{figures/nonglimeiyueshiwu.png} ( The fifteenth day of each lunar month ) \\
\cline{2-2}
& \textbf{Pre-edit:} \includegraphics[height=0.28cm]{figures/panwangqiwang.png} ( Look forward to, Expect ) \\
& \textbf{AdaLoRA:} \includegraphics[height=0.28cm]{figures/wangzhinongli.png} ( ‘\includegraphics[height=0.3cm]{figures/wang.png}’ refers to the fifteenth day of each lunar month ) \\
& \textbf{ROME:} \includegraphics[height=0.27cm]{figures/wangzhinongli2.png} ( \includegraphics[height=0.3cm]{figures/wang.png}: the fifteenth day of each lunar month ) \\
\hline
\multirow{5}*{\textbf{Generalization}}
& \textbf{Rephrase:} \includegraphics[height=0.29cm]{figures/case_generalizaion.png} 
( What does ‘\includegraphics[height=0.3cm]{figures/wang.png}’ mean in the phrase ‘\includegraphics[height=0.3cm]{figures/shidongzhiwangri.png}’ ) \\
& \textbf{Target:} \includegraphics[height=0.29cm]{figures/nonglimeiyueshiwu.png} ( The fifteenth day of each lunar month ) \\
\cline{2-2}
& \textbf{Pre-edit:} \includegraphics[height=0.29cm]{figures/rephrase_pre.png} ( The meaning of \includegraphics[height=0.3cm]{figures/wang.png} refers to observing, expecting, or looking forward to something happening ) \\
& \textbf{AdaLoRA:} \includegraphics[height=0.27cm]{figures/rephrase_lora.png} ( In ancient agricultural culture, ‘\includegraphics[height=0.3cm]{figures/wang.png}’ refers to the fifteenth day of each lunar month ) \\
& \textbf{ROME:} \includegraphics[height=0.30cm]{figures/rephrase_rome.png} ( The meaning of the character \includegraphics[height=0.3cm]{figures/wang.png} here is hope or expectation ) \\
\hline
\multirow{5}*{\textbf{Portability}}
& \textbf{Portability prompt:} \includegraphics[height=0.31cm]{figures/portability.png} 
( Please explain the meaning of ‘\includegraphics[height=0.32cm]{figures/wang.png}’ in ‘\includegraphics[height=0.3cm]{figures/renxvzhiqiu.png}’ ) \\
& \textbf{Target:} \includegraphics[height=0.29cm]{figures/nonglimeiyueshiwu.png} ( The fifteenth day of each lunar month ) \\
\cline{2-2}
& \textbf{Pre-edit:} \includegraphics[height=0.29cm]{figures/portability_pre.png} ( Here, it refers to the sixteenth day of the seventh lunar month ) \\
& \textbf{AdaLoRA:} \includegraphics[height=0.29cm]{figures/portability_lora.png} ( \includegraphics[height=0.3cm]{figures/wang.png}: The fifteenth day of each month ) \\
& \textbf{ROME:} \includegraphics[height=0.28cm]{figures/portability_rome.png} ( The fifteenth day of each lunar month is called \includegraphics[height=0.31cm]{figures/wang.png} ) \\
\hline
\multirow{5}*{\textbf{Locality}}
& \textbf{Locality prompt:} \includegraphics[height=0.32cm]{figures/locality.png} 
( Please explain the meaning of ‘\includegraphics[height=0.32cm]{figures/wang.png}’ in ‘\includegraphics[height=0.3cm]{figures/wuchang.png}’ ) \\
& \textbf{Target:} \includegraphics[height=0.29cm]{figures/xiangyuanchuwang.png} ( To look into the distance ) \\
\cline{2-2}
& \textbf{Pre-edit:} \includegraphics[height=0.28cm]{figures/locality_pre.png} ( The meaning of ‘\includegraphics[height=0.3cm]{figures/wang.png}’ here is to look or to gaze into the distance ) \\
& \textbf{AdaLoRA:} \includegraphics[height=0.3cm]{figures/locality_lora.png} ( The meaning of ‘\includegraphics[height=0.3cm]{figures/wang.png}’ is to look or to gaze into the distance ) \\
& \textbf{ROME:} \includegraphics[height=0.3cm]{figures/locality_rome.png} ( Here, the meaning of ‘\includegraphics[height=0.3cm]{figures/wang.png}’ is to look into the distance ) \\
\hline
\bottomrule
\end{tabular}
}
\end{center}
}
\caption{ We mark correct/wrong responses in \color{green}{green} \color{black}{/} \color{red}{red}.}
\label{tab:case_study}
\end{table*}

==> Table/results_baichuan2_7b.tex <==

\begin{table*}
{
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{3pt}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lrcccc}
% \hline
\toprule
\textbf{Knowledge Type} & \textbf{Method}  
& \textbf{Edit Success}$\uparrow$ & \textbf{$\text{Portability}$}$\uparrow$ & \textbf{Locality}$\uparrow$ & \textbf{Fluency}$\uparrow$ \\ 

\midrule
\multirow{4}{*}{\textbf{Ancient Poetry}}      
& FT-M & 75.70 & 45.15 & - & 456.35 \\ 
& AdaLoRA & 98.16 & 49.31 & - & 362.22  \\ 
& ROME &  &  & - &  \\ 
& GRACE &  &  & - &   \\ 

\midrule 
\multirow{4}{*}{\textbf{Proverbs}}     
& FT-M & 41.19 & 32.05 & - & 427.31 \\ 
& AdaLoRA & 90.43 & 30.01 & - & 319.47  \\ 
& ROME &  &  & - &  \\ 
& GRACE &  &  & - &   \\ 

\midrule 
\multirow{4}{*}{\textbf{Idioms}}      
& FT-M & 49.56 & 35.45 & - & 435.33\\ 
& AdaLoRA & 98.75 & 36.47 & - & 382.52  \\ 
& ROME &  &  & - &  \\ 
& GRACE &  &  & - &   \\ 

\midrule 
\multirow{4}{*}{\textbf{Phonetic Notation}}
& FT-M & 50.08 & 41.99 & 65.00 & 444.20\\ 
& AdaLoRA & 96.02 & 60.22 & 41.71 & 311.13  \\ 
& ROME &  &  &  &  \\ 
& GRACE &  &  &  &   \\ 

\midrule 
\multirow{4}{*}{\textbf{Classical Chinese}}     
& FT-M & 51.17 & 34.24 & 57.06 & 395.05\\ 
& AdaLoRA & 95.43 & 44.35 & 33.90 & 206.47  \\ 
& ROME &  &  & - &  \\ 
& GRACE &  &  & - &   \\ 

\midrule 
\multirow{4}{*}{\textbf{Grographical Knowledge}}     
& FT-M &  &  & - & \\ 
& AdaLoRA &  &  & -  &   \\ 
& ROME &  &  & - &  \\ 
& GRACE &  &  & - &   \\ 

\midrule
\multirow{4}{*}{\textbf{Ruozhiba}}       
& FT-M & 42.53 & 34.65 & 91.85 & 423.63\\ 
& AdaLoRA  & 87.26 & 39.90 & 68.29 & 428.72 \\ 
& ROME &  &  &  &  \\ 
& GRACE &  &  &  &   \\ 


\bottomrule
\end{tabular}
}
}
\caption{Results of some knowledge editing methods on the CKnowEdit on the Baichuan2-7b-chat model.}
\label{tab:experimental_analysis_baichuan}
\end{table*}



==> Table/results_qwen_1_8b.tex <==
\begin{table*}[ht]
{
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{3pt}
\small
\begin{center}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lrcccc}
\toprule
\textbf{Knowledge Type} & \textbf{Method}  
& \textbf{Edit Success}$\uparrow$ & \textbf{$\text{Portability}$}$\uparrow$ & \textbf{Locality}$\uparrow$ & \textbf{Fluency}$\uparrow$ \\ 
\midrule
\multirow{4}{*}{\textbf{Ancient Poetry}}      
& FT-M &26.53  &19.84  &-  &404.87 \\ 
& AdaLoRA &88.10  &22.09  &-  &381.55  \\ 
& ROME &12.35  &12.69  &-  &438.02  \\ 
& GRACE &81.81  &19.72  &-  &380.78   \\ 
& WISE &38.91 &21.70 &- &343.90 \\

\midrule 
\multirow{4}{*}{\textbf{Proverbs}}     
& FT-M &24.48  &21.81  &-  &385.97 \\ 
& AdaLoRA &69.20  &26.76  &-  &328.93  \\ 
& ROME &12.25  &11.13  &-  &471.04  \\ 
& GRACE &58.96  &21.57  &-  &354.09   \\ 
& WISE &33.30 &27.57 &- &326.73 \\

\midrule 
\multirow{4}{*}{\textbf{Idioms}}      
& FT-M &29.33  &22.79  &-  &415.95 \\ 
& AdaLoRA &76.02  &25.78  &-  &393.54  \\ 
& ROME &9.91  &9.24  &-  &436.37  \\ 
& GRACE &66.53  &23.06  &-  &450.78   \\ 
& WISE &39.37 &30.72 &- &317.57 \\

\midrule 
\multirow{4}{*}{\textbf{Phonetic Notation}}
& FT-M &36.26  &31.62  &33.60  &404.81 \\ 
& AdaLoRA &84.64  &41.05  &33.95  &332.02  \\ 
& ROME &16.91  &17.41  &16.33  &455.10  \\ 
& GRACE &80.03  &31.72  &33.68  &363.07   \\ 
& WISE &53.70 &31.00 &29.46 &289.00 \\

\midrule 
\multirow{4}{*}{\textbf{Classical Chinese}}     
& FT-M &23.41  &21.46  &19.88  &394.74 \\ 
& AdaLoRA &49.03  &32.43  &18.28  &221.81  \\ 
& ROME &15.64  &14.36  &14.12  &438.17  \\ 
& GRACE &35.53  &24.56  &29.05  &269.92   \\ 
& WISE &34.65  &24.92  &19.51  &192.51  \\

\midrule 
\multirow{4}{*}{\textbf{Grographical Knowledge}}     
& FT-M &26.50  &22.94  &-  &352.63 \\ 
& AdaLoRA &58.92  &22.44  &-  &229.94  \\ 
& ROME &12.06  &11.64  &-  &427.87  \\ 
& GRACE &50.55  &22.09  &-  &306.88   \\ 
& WISE &48.81 &21.34 &- &114.35 \\

\midrule
\multirow{4}{*}{\textbf{Ruozhiba}}       
& FT-M &28.40  &30.33  &27.79  &405.53 \\ 
& AdaLoRA &96.06  &35.54  &31.71  &428.86  \\ 
& ROME &20.17  &18.28  &20.07  &416.82  \\ 
& GRACE &52.33  &31.02  &27.97  &527.20   \\ 
& WISE &40.37 &36.64 &37.68 &394.42 \\
\bottomrule
\end{tabular}
}
\end{center}
}
\caption{Results of some knowledge editing methods on the CKnowEdit on the Qwen-1.8b-chat model.
The symbol $\uparrow$ indicates that higher numbers correspond to better performance, while $\downarrow$ denotes the opposite, with lower numbers indicating better performance. }
\label{tab:experimental_analysis_qwen_1_8b}
\end{table*}


==> Table/results_qwen_7b.tex <==

\begin{table*}[ht]
{
\small
\begin{center}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lrcccc}
% \hline
\toprule
\textbf{Knowledge Type} & \textbf{Method}  
& \textbf{Edit Success}$\uparrow$ & \textbf{$\text{Portability}$}$\uparrow$ & \textbf{Locality}$\uparrow$ & \textbf{Fluency}$\uparrow$ \\ 

\midrule
\multirow{4}{*}{\textbf{Ancient Poetry}}      
& FT-M &35.41  &21.78  &-  &462.39 \\ 
& AdaLoRA &74.93  &22.17  &-  &428.34  \\ 
& ROME &24.52  &17.39  &-  &439.90  \\ 
& GRACE &52.93  &20.60  &-  &403.19   \\ 
& WISE &43.85 &23.84 &- &329.40 \\

\midrule 
\multirow{4}{*}{\textbf{Proverbs}}     
& FT-M &26.96  &23.38  &-  &433.75 \\ 
& AdaLoRA &75.75  &25.42  &-  &598.61  \\ 
& ROME &10.56  &9.73  &-  &419.54  \\ 
& GRACE &61.83  &23.48  &-  &292.56   \\ 

\midrule 
\multirow{4}{*}{\textbf{Idioms}}      
& FT-M &32.31  &24.53  &-  &448.76 \\ 
& AdaLoRA &71.15  &26.35  &-  &596.30  \\ 
& ROME &11.18  &11.15  &-  &430.01  \\ 
& GRACE &69.24  &23.25  &-  &381.83   \\ 

\midrule 
\multirow{4}{*}{\textbf{Phonetic Notation}}
& FT-M &36.81  &31.49  &38.12  &478.62 \\ 
& AdaLoRA &88.02  &44.81  &48.87  &583.25  \\ 
& ROME &16.20  &15.74  &15.72  &400.22  \\ 
& GRACE &82.96  &30.23  &36.31  &353.90   \\ 

\midrule 
\multirow{4}{*}{\textbf{Classical Chinese}}     
& FT-M &20.43  &21.57  &23.29  &445.51 \\ 
& AdaLoRA &51.17  &31.50  &20.31  &270.58  \\ 
& ROME &22.04  &18.88  &18.49  &420.11  \\ 
& GRACE &33.03  &21.83  &22.42  &268.91   \\ 

\midrule 
\multirow{4}{*}{\textbf{Grographical Knowledge}}     
& FT-M &28.41  &27.44  &-  &439.34 \\ 
& AdaLoRA &62.75  &25.73  &-  &432.39  \\ 
& ROME &15.02  &13.98  &-  &382.19  \\ 
& GRACE &58.16  &27.41  &-  &315.66   \\ 

\midrule
\multirow{4}{*}{\textbf{Ruozhiba}}       
& FT-M &28.38  &30.54  &30.16  &437.44 \\ 
& AdaLoRA &97.03  &34.67  &33.25  &429.64  \\ 
& ROME &21.90  &20.30  &24.31  &434.07  \\ 
& GRACE &79.46  &30.37  &30.58  &451.01   \\ 
\bottomrule
\end{tabular}
}
\end{center}
}
\caption{Results of some knowledge editing methods on the CKnowEdit on the Qwen-7b-chat model. The symbol $\uparrow$ indicates that higher numbers correspond to better performance, while $\downarrow$ denotes the opposite, with lower numbers indicating better performance. }
\label{tab:experimental_analysis_qwen-7b}
\end{table*}



==> section/Background.tex <==
\section{Background: Knowledge Editing}

Pioneered by \citet{DBLP:conf/emnlp/CaoAT21}, knowledge editing is designed to correct factual inaccuracies or update specific facts in a model without the need for comprehensive retraining. This approach is particularly appealing as it allows for the rectification of errors while maximizing the preservation of unrelated knowledge, thus maintaining the overall integrity and performance of the model.

The process of knowledge editing involves identifying a specific input-output pair, denoted as an edit descriptor $(x_e,y_e)$, where the current model's prediction $f_\theta(x_e)$ does not align with the desired output $y_e$. The objective is to modify the model's parameters from $\theta$ to $\theta_e$ such that the edited model $f_{\theta_{e}}$ accurately predicts the target output for the given input, i.e., $f_{\theta_{e}}(x_e)=y_e$. This transformation is achieved by concatenating the edit descriptor and then optimizing the model to maximize the conditional probability of the target output given the input, formally defined as:
\[
{\theta}_e = \operatorname{argmax}_{\theta} P(y_e | x_e; \theta)
\]
The significance of knowledge editing lies in its precision and efficiency. Unlike full retraining, which can be computationally expensive and time-consuming, knowledge editing focuses on making minimal yet impact changes to the model's parameters. This targeted approach ensures that the model's performance on unrelated tasks remains unaffected, thereby preserving the vast knowledge and skills the model has acquired during its initial pre-training phase.

==> section/Construction.tex <==
\section{CKnowEdit Dataset Construction}
\textbf{CKnowEdit} is meticulously designed to more deeply discern the nuances and challenges inherent in the comprehension of the Chinese language by current LLMs, providing a robust resource for refining Chinese-specific knowledge within LLMs.
All data utilized in the construction of this dataset is derived from publicly available sources on the Internet, ensuring that there are no copyright or intellectual property risks involved. 
The procedures employed in the creation of \textbf{CKnowEdit} and the associated statistical details are outlined in Figure \ref{fig:construction}.
% \subsection{Dataset Construction}

We delve into diverse and authentic Chinese linguistic resources, including the rich tapestry of classical literature, the vibrant expressions of contemporary colloquial speech, and the unique cultural insights found within the Baidu Tieba forum known as Ruozhiba, each reflecting distinct facets of Chinese linguistic identity.
Particularly, we select the common misunderstandings and cultural misinterpretations found in current large language models (Qwen-7B-Chat\footnote{\url{https://huggingface.co/Qwen/Qwen-7B-Chat}}) and build the editing dataset that targets these specific knowledge gaps. 
The construction process also includes a \textbf{human review} phase to verify the accuracy and relevance of the information, thereby ensuring that the edits made to the model's knowledge base are reasonable and faithful.
The details of construction for each type of knowledge are as follows:

\paragraph{Chinese Literary Knowledge.}
This kind of knowledge in CKnowEdit includes \textbf{Ancient Poetry}\footnote{\url{https://zhuanlan.zhihu.com/p/414484867}}, \textbf{Proverbs}\footnote{\url{http://www.360doc.com/content/19/0218/14/39098269_815762159.shtml}, \url{http://www.360doc.com/content/19/0312/16/5784427_820995624.shtml}, \url{http://www.360doc.com/content/19/0126/14/55773589_811408910.shtml}} and \textbf{Idioms}. 
The selection process involves identifying segments of text that commonly present challenges for language models, focusing on those that require a deep understanding of cultural context, historical significance, or linguistic detail.
These materials are drawn from reputable educational sources and cultural repositories, reflecting China's rich educational standards and profound heritage.
For example, ancient poetry and proverbs are sourced from well-recognized compilations commonly used in school curricula, such as the ``Must-memory ancient poems for college entrance examination'' for ancient poetry while idioms and phonetic notations are derived from collections known for their extensive usage and occasional misinterpretations, such as the ``Common error-prone idioms and error-prone pronunciations'' collection.
Each category has been developed to address specific errors of biases in language understanding by LMs.
For example, classical Chinese entries focus on polysemy and contextual meanings, which are often challenging for LLMs. 
% The entries for idioms and phonetic notations target common inaccuracies in interpretation and pronunciation. 
% The entries within each category are initially generated by querying the Qwen-7b-chat model \cite{bai2023qwen}. 

We initially obtain the generated texts by posing questions to the Qwen-7b-chat model \cite{bai2023qwen} and collecting their responses.
Then we collect the original prompt, the model’s incorrect response, and the accurate answer. 
The accurate answers are generated through GPT-4 (\textit{gpt-4-turbo-2024-04-09}) \cite{achiam2023gpt}, utilizing human-crafted prompt templates designed to ensure the correction's relevance and applicability.
Each entry is then reviewed by humans, who correct the misinterpretations or misrepresentations in the entries given by the GPT-4 model. 
The annotation process depends on the online Chinese dictionary\footnote{\url{https://zd.hwxnet.com/}} to ensure the knowledge is reliable. 

\paragraph{Chinese Linguistic Knowledge.}
In Chinese, certain words exhibit multiple phonetic notations or meanings depending on their usage within different contexts. 
Similarly, the word may appear in various Classical Chinese sentences with different meanings, necessitating precise contextual understanding to ensure accurate interpretation.
To address these nuances, the dataset includes entries where the same word appears in different sentences or phrases, requiring distinct phonetic annotations or interpretations. 
This part contains two parts: \textbf{Phonetic Notation}\footnote{\url{https://zhuanlan.zhihu.com/p/599709230}}, and \textbf{Classical Chinese}\footnote{\url{https://zhuanlan.zhihu.com/p/622859964}, \url{https://www.bilibili.com/read/cv20279857/}}
The construction part is the same as the literary knowledge, but additional human review steps are taken to generate entries for portability and locality since there are too many errors in the data entries generated by the GPT-4 model (likely because the knowledge about the usage of these languages in the GPT-4 model is also wrong.) 
For portability, entries are crafted to test if the language model can apply these distinctions across different scenarios, thereby understanding that a change in one instance should reflect correctly in similar uses.
For locality, the dataset ensures that changes made to the word's phonetic notation or meaning in one context do not erroneously alter its correct applications in others where its pronunciation or meaning should remain different. 
% Portability entries are created to ensure that the corrections made to one instance of a term or expression would appropriately influence related terms or expressions within the dataset.
% This involves generating related prompts that might use different phrases or contexts but still require the model to apply the same corrected understanding.
% Locality entries are developed to confirm that the corrections do not inadvertently alter the correct understanding or representation of other unrelated data. 
% This is crucial for maintaining the overall integrity and utility of the model, ensuring that enhancements in one area do not lead to degradation in another.



% This is crucial in maintaining the integrity and utility of the language model across diverse linguistic tasks, ensuring that enhancements in understanding specific cases do not compromise the overall accuracy and functionality of the model.

\input{Table/main_table}

\paragraph{Chinese Geographical Knowledge.}
The \textbf{Geographical Knowledge} dataset is carefully designed to correct and refine geographical commonsense data within language models, emphasizing the importance of accurate and contextually relevant geographical information.
% This dataset originates from an identified need to address common geographical inaccuracies and update outdated information within AI systems.
The dataset is built upon a series of prompts which is human-crafted with specific geographical knowledge from Internet\footnote{\url{https://baijiahao.baidu.com/s?id=1682950669904608106&wfr=spider&for=pc}, \url{https://www.sohu.com/a/419822319_100941}, \url{https://www.jingyanben.com/qitawendang/125282.html?page=1}, \url{https://www.sohu.com/a/412325688_281347}, \url{http://www.360doc.com/content/20/0613/11/7254176_918223750.shtml}}. 
The incorrect answers provided by the model are documented. 
Each corresponding correct answer is sourced from reliable, authoritative texts.
Each dataset entry consists of the original geographical prompt, the incorrect response from the Qwen-7b-chat model, and the correct answer. 
For each pair of prompts and responses, GPT-4 is employed again to generate additional prompts testing the LM's ability to apply the corrected information in different but related contexts. 
For example, two-step logical reasoning about the knowledge of the position in the correct answer. 
After the initial generation and correction with the help of GPT-4, each entry undergoes a human review process to refine the language and ensure the accuracy of the geographical data.
This step is vital for validating the portability, making sure they align with the core factual correction and enhance the overall utility of the dataset.

\paragraph{Chinese Ruozhiba.}
The \textbf{Ruozhiba} \cite{bai2024coigcqia} dataset is constructed from a subsection of Baidu Tieba known as Ruozhiba, which is famed for being a breeding ground for original, often humorous content that incorporates logical puzzles and philosophical musings. 
These characteristics make it an invaluable resource because the data in it requires not just linguistic understanding, but also the capability to handle logical traps. 
In order to collect the knowledge that the LLM incorrectly has, the selected Ruozhiba dataset content is the question sentences that typically include logical traps or require higher-order thinking to interpret correctly. 
% This source is available at GitHub repository\footnote{\url{https://github.com/Leymore/ruozhiba}}.

Each selected question is used as a prompt in interactions with both the Qwen-7b-chat and GPT4 models.
Then we collect the responses: where Qwen-7b-chat falters, typically providing incorrect or logically inconsistent answers, and where GPT-4 succeeds in delivering accurate responses. 
For each pair of prompts and responses, the GPT-4 is employed again to generate structured dataset entries with a prompt template that focuses on portability and locality. 
Portability involves creating additional prompts and answers that extend the application of the corrected knowledge to similar or related scenarios, testing the model's ability to generalize the new information. 
And locality ensures that the corrections do not inadvertently affect the correct understanding of other unrelated pieces of knowledge. 
The last phase is a human review process to ensure that each entry is accurate by deleting the wrong data entry generated by GPT-4. Meanwhile, human review also helped correct some JSON format errors, as well as a small number of factual inaccuracies, ensuring that the final version of the constructed dataset is error-free.




